A First Look at Deep Learning Apps on Smartphones

We are in the dawn of deep learning explosion for smartphones. To bridge the gap between research and practice, we present the first empirical study on 16,500 the most popular Android apps, demystifying how smartphone apps exploit deep learning in the wild. To this end, we build a new static tool that dissects apps and analyzes their deep learning functions. Our study answers threefold questions: what are the early adopter apps of deep learning, what do they use deep learning for, and how do their deep learning models look like. Our study has strong implications for app developers, smartphone vendors, and deep learning R\&D. On one hand, our findings paint a promising picture of deep learning for smartphones, showing the prosperity of mobile deep learning frameworks as well as the prosperity of apps building their cores atop deep learning. On the other hand, our findings urge optimizations on deep learning models deployed on smartphones, the protection of these models, and validation of research ideas on these models.

==> secs/implication.tex <==
\section{Implications}\label{sec:implications}

\note{can be expanded and merged into each section}

The key observation made in this work is that DL has been already adopted in many in-the-wild smartphone apps, and the number of such apps is increasing sharply.
This result justifies future investment in the field of mobile DL.
With our study as the endorsement, researchers are better motivated to focus on optimizing the runtime performance of mobile DL, e.g., latency, energy, and security.
For example, there's emergent demand to build a tool that can help protect mobile DL models from being stolen, either in system-level or app-level, since we find that currently most DL models are exposed without protection and the existing DL frameworks rarely support such protection mechanism.
Similarly, our study may endow developers, especially those individuals or small companies, with more confidence in deploying DL on their products. This is because our analysis has shown that the developers of popular apps have already made the attempt, and the role played by DL in their popular apps is essential rather than dispensable.
On the other hand, however, the potential of DL is far from being fully utilized. The models used are very lightweight and few of them are well optimized. It leaves researchers and developers a lot of space to explore how DL can really change the mobile intelligence.

Our analysis results demonstrate that in-the-wild DL models are very lightweight compared to classical DL models. This finding is insightful to future research efforts on mobile DL. In fact, according to our observation, most existing research efforts are motivated and validated on classical DL models, e.g., VGG. This may hurt the practicality and generality of their contributions. We advocate that novel DL frameworks/toolkits/schemes in the future shall be also validated on those in-the-wild models as well.

Our findings also provide useful guidance for developers on how to properly deploy DL on their apps.
As demonstrated, mobile-oriented DL frameworks do better in reducing the size of library and models compared to the generous-purpose ones. This advantage has also been noticed by developers, with increasing adoption of those mobile-oriented frameworks such as \emph{TFLite} and \emph{ncnn} in real apps.

==> secs/tab_checkin.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\large
\begin{tabular}{l|l|l|}
\cline{2-3}
 & \cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}l@{}}DL apps in\\ Jun. 2018\end{tabular}}} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}l@{}}non-DL apps\\ in Jun. 2018\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}l@{}}DL apps in\\ Sep. 2018\end{tabular}}}} & 142 & 48 (check-in) \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}l@{}}non-DL apps\\ in Sep. 2018\end{tabular}}}} & 5 (check-out) & 11,705 \\ \hline
\end{tabular}
\caption{The check-in and check-out of DL on mobile apps.}
\label{tab:checkin}
\end{table}

==> secs/tab_term.tex <==
\begin{table}[]
\small 
\begin{tabular}{l|l}
\hline
\textbf{Term} & \textbf{Definition} \\\hline
DL & deep learning \\
DL apps & apps that use DL for specific functionality \\
non-DL apps & all apps excluding DL apps \\
% DL-apks & Android apk files of DL apps \\
DL libs & native libraries (.so) that implement the DL \\
& functionality, i.e., prediction and (optional) training \\
non-DL libs & all native libraries excluding DL libs \\
DL models & model files that contain the structures and parameters \\
& of DL algorithm \\
DL frameworks & frameworks/libraries who really implement the DL \\
& functionality, i.e., training and prediction.\\\hline
\end{tabular}
\caption{Terminology used in this paper. XXXX this table can be deleted. Looks like we don't have to diff DL libs and frameworks XXX }
\label{tab:term}
\end{table}
